SpellBound: Defending Against Package Typosquatting

Package managers for software repositories based on a single programming language are very common. Examples include npm (JavaScript), and PyPI (Python). These tools encourage code reuse, making it trivial for developers to import external packages. Unfortunately, repositories' size and the ease with which packages can be published facilitates the practice of typosquatting: the uploading of a package with name similar to that of a highly popular package, typically with the aim of capturing some of the popular package's installs. Typosquatting has serious negative implications, resulting in developers importing malicious packages, or -- as we show -- code clones which do not incorporate recent security updates. In order to tackle this problem, we present SpellBound, a tool for identifying and reporting potentially erroneous imports to developers. SpellBound implements a novel typosquatting detection technique, based on an in-depth analysis of npm and PyPI. Our technique leverages a model of lexical similarity between names, and further incorporates the notion of package popularity. This approach flags cases where unknown/scarcely used packages would be installed in place of popular ones with similar names, before installation occurs. We evaluated SpellBound on both npm and PyPI, with encouraging results: SpellBound flags typosquatting cases while generating limited warnings (0.5% of total package installs), and low overhead (only 2.5% of package install time). Furthermore, SpellBound allowed us to confirm known cases of typosquatting and discover one high-profile, unknown case of typosquatting that resulted in a package takedown by the npm security team.

==> threat_model.tex <==
\section{Threat Model}

Packages created and maintained by the community are the lifeblood
of any package repository. Consequently, the process of uploading
packages is optimized for speed and simplicity in order to
minimize the burden on package developers and incentivize package
creation in general. Malicious package developers are not exempt.
All users are welcome to create and upload any number of packages
at no cost.

The contents of these packages are just as flexible. Users are
able to add arbitrary code to their packages. However, packages
are not limited to containing pure source code. Packages on npm
are free to consist of shell scripts, program binaries, and more.
This feature creates a double-edged sword. It allows
for the creation of more powerful tools and more powerful exploits.
At installation time, malicious packages could execute shell scripts
by using npm's popular scripting features. Historical examples of
malicious packages that chose to take this route attempted to remove
all files on the user's computer, download files from remote servers,
or SSH into machines which presumably were under the attacker's control.
Other malicious packages have taken more subtle routes by
executing their payload at run time, rather than during installation.

Transparency is a staple of modern package repositories. This gives
users the ability to see exactly what code is being executed on their
machines. However, this fundamental transparency can be used by
attackers to create more elaborate typosquatting attacks. The name,
popularity (in terms of weekly downloads), and source code for every
package on the repository are publicly available. With no restrictions on
package name similarity, adversaries could theoretically create malicious
packages covering every possible typo of a popular package name.

Naive typosquatters could find an incredibly popular package and upload
a purely malicious package under an incredibly similar name. Other
developers who make this typo during installation, although they would be
compromised, may figure this out relatively quickly, since their desired
functionality isn't present. More experienced typosquatters could
anticipate this. To counteract this, attackers could copy and reupload
the source code of the package they are targeting with their payload
added. This would serve a dual-purpose of infecting users and remaining 
undetected for extended periods of time since, to the end user, the package
behaves as expected.

Because of the complex and interconnected web of dependencies present in
package repositories, typosquatting attacks target more than inaccurate typists.
A well-intentioned package creator could add a dependency to their package,
make a typo, and fall victim to a typosquatting attack. Beyond that, all
users who install that developers package will be served the malicious package.
Despite making no mistakes during the installation process, the package
manager will serve these users a typosquatting package. When installing
packages with dozens, or even hundreds, of transitive dependencies, end users are
implicitly trusting package developers to vet their packages for vulnerable
or malicious code. Furthermore, the consumers of any application that depends
on typosquatting package could be affected.

The motivation of those perpetrating typosquatting attacks can vary. Some adversaries
could do this simply to waste time, confuse, or frustrate package repository users. Others
conducting these attacks could have financial motivations and plant cryptocurrency
miners in their typosquatting packages. Information theft could be another motivation,
as a number of malicious npm packages capable of stealing user information and uploading
it to a remote server have been removed from the repository. Attackers could also
have bigger plans, and use typosquatting as a tool to create a botnet capable of
denial-of-service attacks.
